Text-to-SQL Error Correction with Language Models of Code

Despite recent progress in text-to-SQL parsing, current semantic parsers are still not accurate enough for practical use. In this paper, we investigate how to build automatic text-to-SQL error correction models. Noticing that token-level edits are out of context and sometimes ambiguous, we propose building clause-level edit models instead. Besides, while most language models of code are not specifically pre-trained for SQL, they know common data structures and their operations in programming languages such as Python. Thus, we propose a novel representation for SQL queries and their edits that adheres more closely to the pre-training corpora of language models of code. Our error correction model improves the exact set match accuracy of different parsers by 2.4-6.5 and obtains up to 4.3 point absolute improvement over two strong baselines. Our code and data are available at https://github.com/OSU-NLP-Group/Auto-SQL-Correction.

==> old_content.tex <==
% \section{Error Analysis}
% \label{appendix:error}

% \begin{table}[t]
% \small
% %\renewcommand{\arraystretch}{1.1}
% \centering
% \begin{tabular}{lccc}
% \toprule
% \textbf{Error Category} & \textbf{Resolved} & \textbf{Unresolved} & \textbf{All}\\
% \midrule
% Table/Column Error & 10 & 24 & 34 \\
% Value Error & 4 & 5 & 9 \\
% Operand Error & 1 & 6 & 7 \\ 
% Join Error & 2 & 9 & 11 \\
% Inter-Clause Error & 1 & 6 & 7 \\
% Subquery Error & 2 & 17 & 19\\
% Initial Parse Error & 1 & 4 & 5\\
% \midrule
% False Positive & - & - & 7\\
% Annotation Error & - & - & 1\\
% \midrule
% Total & 21 & 71 & 100\\
% \bottomrule
% \end{tabular}
% \caption{\label{tab:error} Analysis of 100 SmBoP errors in Spider development set. We group the errors into 9 categories and examine if our CodeT5-PyDict-Program model resolves them. }
% \end{table}

% We define each category of SQL parsing errors (Table \ref{tab:error}) as follows:
% \begin{itemize}
%     \item Table/Column Error: The parse has some incorrect table names and/or column names. 
%     \item Value Error: The parse has wrong values in its conditional expressions. 
%     \item Operand Error: The unary/binary operands on two columns or the aggregation functions have errors. 
%     \item Join Error: The tables in the parse and their joining conditions have some errors. 
%     \item Inter-Clause Error: The parse has some extra/missing clauses, or the clause need to be replaced with another. 
%     \item Subquery Error: The parse has some errors in the subquery, or the subquery is missing. 
%     \item Initial Parse Error: The base text-to-SQL parser generated an incomplete and/or ungrammatical SQL. In this case, the error correction model needs to generate the correct parse from almost scratch.  
%     \item False Positive: The parse is semantically correct. This is usually caused by the ``distinct'' keyword. 
%     \item Annotation Error: The annotated parse is incorrect. 
% \end{itemize}
% Through careful analysis of 100 errors sampled from SmBop (Section \ref{results}), our findings are as follows:

% \paragraph{Our model's generation results are highly consistent.}
% Since our model is generating both edit actions and their resulting SQL query, we examine if they are consistent so that we can convert the wrong SQL query to the final prediction by applying the edit actions manually. 
% Based on our analysis, we find that our model generates programs that are consistent with the resulting queries for 97 out of 100 test examples.
% According to the evaluations in \citet{ZhangETAL22CoditT5} on other tasks ($88-92\%$ on bug fixing), $97\%$ is a decent performance on generation consistency.
% However, this high consistency is also because our model would sometimes assign higher probabilities to programs that copy from the input than the correct programs. 
% We identify this problem as an important future direction to improve our model. 

% \paragraph{Grounding is the major source of errors.}
% We found that incorrect grounding natural language utterances to database content is the main cause of text-to-SQL errors (Table/Column Error and Value Error), and our model successfully resolves 14 out of 43 such errors in our analysis.
% We hypothesize that our model effectively leverages the correct clauses in the  wrong SQL query as its editing context.
% However, we noticed that 29 more examples are still unresolved, leaving substantial room for further improvement.
% As a future direction, we can incorporate our model into an interactive semantic parsing framework and suggest candidate table names and column names for users to choose from. 
% By interacting with end users, our model would be able to resolve more errors.

% \paragraph{Clause-level errors are hard to correct.}
% Clause-level errors (Inter-Clause Error and Subquery Error) are also very frequent in our analysis. 
% For subquery errors, we found that they usually involve multiple clauses in the subquery, and our model can only correct the first few of them. 
% We emphasize this is a strong rationale for us to combine our model with an interactive framework in the future.
% By interacting with users to correct one clause at a time, our model would suffer less from common sequence-to-sequence generation issues, such as memorization and handling long sequences.
% Thus, it would be able to fully resolve more errors that require multiple edit steps. 

% \paragraph{Better representations for database schema are needed. } 
% When analyzing Join errors, we found that our current representation for database schemas is missing critical information, such as foreign keys, for our error correction model to infer Join relations.
% Following the sucssess of our PyDict representation for SQL, we hypothesize that we can also design a code representation for database schemas and include such information. 
% With this new representation, we expect language models of code would better understand the schema and correct more Join relations successfully.

% \begin{table*}
% \small
% %\setlength{\tabcolsep}{4pt}
% %\renewcommand{\arraystretch}{1.2}
% \centering
% \begin{tabular}{lcccccccc}
% \toprule
% \multirow{2}{*}{\textbf{Models}} & \multirow{2}{*}{\textbf{Query}} & \multirow{2}{*}{\textbf{Edit}} & \multicolumn{2}{c}{\textbf{CodeT5}} & \multicolumn{2}{c}{\textbf{BRIDGEv2}} & \multicolumn{2}{c}{\textbf{SmBoP}} \\
% \cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}
%  & & & EM & EX & EM & EX & EM & EX\\
% \midrule
% \multirow{3}{*}{CoditT5} & SQL & Token-level & 4.4 (0.2) & 2.2 (0.6) & -15.6 (1.6) & -5.1 (0.8) & -1.4 (1.8) & 0.1 (0.5) \\
%  & SQL & Clause-level & 11.5 (1.2) & 5.1 (1.3) & 4.1 (1.8) & 8.5 (0.7) & 6.6 (0.2) & 7.7 (1.3) \\
%  & PyDict & Clause-level & 11.9 (0.4) & 7.9 (1.1) & 1.6 (2.8) & 7.5 (2.6) & 6.7 (1.1) & 7.1 (1.0) \\
% \midrule
% \multirow{3}{*}{CodeT5} & SQL & Token-level & 10.7 (2.3) & 6.3 (1.3) & -6.3 (1.2) & 3.7 (2.4) & 3.9 (1.5) & 4.7 (2.5) \\
%  & SQL & Clause-level & 15.0 (0.8) & \underline{12.6} (1.7) & 5.7 (1.3) & 13.5 (0.6) & 8.2 (2.2) & 8.4 (1.2)  \\
%  & PyDict & Clause-level & 10.4 (2.1) & 9.5 (2.2) & 6.2 (1.1) & 13.3 (0.7) & 10.7 (2.3) & \underline{10.1} (1.0) \\
% \midrule
% CodeT5$^*$ & \multirow{2}{*}{PyDict} & \multirow{2}{*}{Program} & \textbf{17.3} (1.0) & \textbf{13.3} (0.5) & \textbf{8.0} (1.3) & \textbf{15.5} (0.7) & \underline{10.8} (1.6) & 9.3 (2.6) \\
% CodeT5 &  &  & \underline{16.8} (0.6) & \underline{12.6} (0.2) & \textbf{8.0} (0.8) & \underline{15.0} (2.0) & \textbf{13.6} (1.4) & \textbf{12.8} (1.3) \\
% \bottomrule
% \end{tabular}
% \caption{\label{tab:errRate}
% Exact Set Match (EM) and Execution Match (EX) error reduction rate on Spider development set. The \textbf{best performances} are in bold and the \underline{second best ones} are underlined. $^*$We fine-tune the model to generate edit programs only (without resulting queries) and use Python interpreter to execute the edit actions. 
% }
% \end{table*}

% In addition to results in Section \ref{results}, we also present the zero-shot perplexity of different representations on CoditT5 (Figure \ref{fig:ppl_coditT5}). 
% From Table \ref{tab:main}, we also find that \textbf{CoditT5 may be overfitting to its pre-training data}. 
% Albeit CoditT5 is a language model for code editing, we found that it constantly underperforms CodeT5 across three representations. 
% In addition, CoditT5 shares the same pre-training corpus, CodeSearchNet \citep{codesearchnet}, with its base language model (CodeT5)\footnote{CodeT5 used pre-training data other than CodeSearchNet, and this diversity may also help with generalization.}.
% So, \textit{the model is pre-trained on the same corpus twice}. 
% For these two facts, we suggest that CoditT5 may be overfitting to its pre-training data. 
% As a result, while CoditT5 variants have lower perplexity for edit actions represented with special tokens, they fail to adapt to edit patterns for SQL queries, even if represented in Python dictionaries. 
